Unifying Heterogeneous Electronic Health Records Systems via Text-Based Code Embedding

EHR systems lack a unified code system forrepresenting medical concepts, which acts asa barrier for the deployment of deep learningmodels in large scale to multiple clinics and hos-pitals. To overcome this problem, we introduceDescription-based Embedding,DescEmb, a code-agnostic representation learning framework forEHR. DescEmb takes advantage of the flexibil-ity of neural language understanding models toembed clinical events using their textual descrip-tions rather than directly mapping each event toa dedicated embedding. DescEmb outperformedtraditional code-based embedding in extensiveexperiments, especially in a zero-shot transfertask (one hospital to another), and was able totrain a single unified model for heterogeneousEHR datasets.

==> tex/2RelatedWorks.tex <==
%\section{Related Work}
% \textbf{Neural Text Encoders.}
%Early text embedders encode each word as a vector whose semantic similarity is represented by a distance measure \citep{mikolov2013efficient}.Recently, Bidirectional Encoder Representations from Transformers (BERT) \citep{bert} have shown significant improvements on Natural Language Processing (NLP) tasks. This model employ a unique pre-training strategy, Masked Language Modeling (MLM) and Next Sentence Prediction (NSP), to understand complex relationships within the input text.

% \textbf{this section can be removed} Recent work has indicated that domain-specific pre-training can improve the performance of large language models like BERT, which rely on general domain text such as Wikipedia and BooksCorpus \citep{bookcorpus}. Particularly in the biomedical domain, several studies have developed BERT variants further trained on medical or clinical corpora in order to offer more precise contextualized embeddings for domain-specific tasks. Domain-specific BERT variants in the biomedical field have been continually pre-trained on research articles from PubMed \citep{biobert}, MIMIC-III clinical text \citep{clinicalbert}, or or a combination of the two \citep{bluebert}, and scratch trained on articles from PubMed \citep{pubmedbert}. 

% \noindent \textbf{Representation Learning for Predictive Healthcare.}
%  Models based on autoencoders are used to learn patient representations for downstream prediction tasks \citep{miotto2016deep, che2015deep}. Given the sequential longitudinal EHR data, diverse works have been proposed to learn patient representations using recurrent neural networks (RNN)  to perform accurate prediction, interpretability, or scalability \citep{lipton2015learning, choi2016doctor, choi2016retain, pham2016deepcare, ma2017dipole, rajkomar2018scalable, steinberg2020language}, while other works have focused on learning medical concept representations \citep{choi2016multi, choi2017gram, ma2018kame, choi2018mime, song2019medical, yin2019domain, zhang2020hierarchical}. Other model architectures are also used for predictive healthcare such as gradient boosted machines \citep{chen2019deep}, convolutional nets \citep{nguyen2016deep, landi2020deep}, and Transformer-based models \citep{song2018attend, shang2019pre, choi2020learning, li2020behrt, rasmy2020med}.

% Previous works assumes that medical codes are the basic unit of processing, namely code-based embedding. Our paper focuses on a new problem setting—the unification of heterogeneous code systems in EHR—and therefore sits independent to these previous works. As such, our proposed approach can be combined with prior frameworks for representation learning and predictive modeling.


